CLEAR: Generative Counterfactual Explanations on Graphs

Counterfactual explanations promote explainability in machine learning models by answering the question "how should an input instance be perturbed to obtain a desired predicted label?". The comparison of this instance before and after perturbation can enhance human interpretation. Most existing studies on counterfactual explanations are limited in tabular data or image data. In this work, we study the problem of counterfactual explanation generation on graphs. A few studies have explored counterfactual explanations on graphs, but many challenges of this problem are still not well-addressed: 1) optimizing in the discrete and disorganized space of graphs; 2) generalizing on unseen graphs; and 3) maintaining the causality in the generated counterfactuals without prior knowledge of the causal model. To tackle these challenges, we propose a novel framework CLEAR which aims to generate counterfactual explanations on graphs for graph-level prediction models. Specifically, CLEAR leverages a graph variational autoencoder based mechanism to facilitate its optimization and generalization, and promotes causality by leveraging an auxiliary variable to better identify the underlying causal model. Extensive experiments on both synthetic and real-world graphs validate the superiority of CLEAR over the state-of-the-art methods in different aspects.

==> 2_preliminary.tex <==
\section{Preliminaries}
% \subsection{Counterfactual Explanations on Graphs} 
% It has been 

\subsection{Structural Causal Model}
Pearl's structural causal model (SCM) \cite{pearl2009causality} consists of a \textit{causal graph} and an associated set of \textit{structural equations}. A causal graph is a directed acyclic graph (DAG) with variables represented as nodes, and causal relations between variables represented as directed edges. Structural equations describe the causal relations between variables. SCM can be denoted by a triple $(U,V,F)$: $U$ is a set of exogenous variables, and $V$ a set of endogenous variables. The structural equations $F=\{f_1,...,f_{|V|}\}$, for each $V_i\in V$, its associated structural equation follows the form: $V_i = f_i(\mathtt{PA}(V_i), U_i)$, here $\mathtt{PA}(V_i)$ denotes the set of parent variables of $V_i$, and $U_i\in U$ denotes the parent exogenous variables of $V_i$.

\subsection{Nonlinear Independent Component Analysis}
In nonlinear independent component analysis (ICA) [], it is assumed that the observed $d_x$-dimensional data, $X$, is generated from a smooth and invertible nonlinear transformation of independent latent variables (referred to as \textit{sources}) $Z = (Z_1,...,Z_{d_z})$, where $d_z\leq d_x$. The goal of nonlinear ICA is to recover $Z$ from $X$. Similarly, traditional VAE  models also assume that the observed features $X$ are generated by a set of latent variables $Z$, and learn a generative model $p(X,Z)$ and an inference model $q(Z|X)$ to approximates the posterior $p(Z|X)$. However, a limitation of traditional VAEs is the lack of identifiability of the deep latent-variable model, i.e., we can find different transformations of $Z$ that can lead to the same marginal density $p(X)$. It has been proved that any model with unconditioned $p(Z)$ is unidentifiable. Recently, \cite{khemakhem2020variational} proposes a family of identifiable VAE (iVAE) based on the assumption that the prior distribution $p(Z|U)$ can be conditionally factorized, where $U$ is an 
auxiliary observed variable, e.g., a time index in a time series, or a class label.

\noindent\textbf{Connection between ICA and SCM.} The connection between ICA and SCM has been initially discussed in \cite{shimizu2006linear} for the linear case, and then has been extended to nonlinear cases \cite{monti2020causal}. Generally, a SCM can be considered as a nonlinear ICA model if the exogenous variables in the SCM are seen as the sources in ICA. Even though it has been proven \cite{karimi2020algorithmic} that it is impossible to identify the causal model from data distribution without additional assumptions or prior knowledge of the structural equations and exogenous variables, based on the above connection, the identifiability of the underlying SCM can also be improved with the help of the auxiliary observed variable.  

%\noindent\textbf{Identifiability and Counterfactual.}
% same data -> different SCMs (ICAs) -> different counterfactuals
% auxiliary -> help identify sources & sources -> data -> help better counterfactual

%It has been shown that 
